mmWave-Whisper: Phone Call Eavesdropping and Transcription Using Millimeter-Wave Radar

This paper introduces mmWave-Whisper, a system that demonstrates the feasibility of full-corpus automated speech recognition (ASR) on phone calls eavesdropped remotely using off-the-shelf frequency modulated continuous wave (FMCW) millimeter-wave radars. Operating in the 77-81 GHz range, mmWave-Whisper captures earpiece vibrations from smartphones, converts them into audio, and processes the audio to produce speech transcriptions automatically. Unlike previous work that focused on loudspeakers or limited vocabulary, this is the first work to perform such a speech recognition by handling large vocabulary and full sentences on earpiece vibrations from smartphones. This approach expands the potential of radar-audio eavesdropping. mmWave-Whisper addresses challenges such as the lack of large scale training datasets, low SNR, and limited frequency information in radar data through a systematic pipeline designed to leverage synthetic training data, domain adaptation, and inference by incorporating OpenAI's Whisper automatic speech recognition model. The system achieves a word accuracy rate of 44.74% and a character accuracy rate of 62.52% over a range of 25 cm to 125 cm. The paper highlights emerging misuse modalities of AI as the technology evolves rapidly.

==> sections/platform.tex <==
\section{Platform Description}

% 1. Data collection
% 2. ASR: Finetuning whisper models
% 3. Describe radar platform, GPU and libraries used (Pytorch, librosa, huggingface)

% Platform information:
% Dataset: LibriSpeech
% Phone: Samsung Galaxy S20
% Radar: TI AWR1843 BOOST in 77 GHz (FMCW).
% Libraries: Pytorch, librosa, huggingface
% GPU: NVIDIA Quadro RTX 8000
% Ranges over which the experiments were performed.
% Summary of results.

{\papertitle} is implemented using the Texas Instruments AWR1843 BOOST, which operates in the range of 77-81 GHz and utilizes FMCW signals. The attack is conducted on a Samsung Galaxy S20. Radar sensor data is pre-processed offline using MATLAB and Python modules before being fed into machine learning models implemented with HuggingFace Transformers and PyTorch for ASR. The models are trained on an NVIDIA Quadro RTX 8000 GPU. The ASR model employed is OpenAI's Whisper-large-v2, which is a SOTA ASR model. %{\color{red}The system achieves a word recognition accuracy of 40\% and a character recognition accuracy of 60\% over a distance of 0.25 to 1.5 meters. -- remove this or change it.}

\begin{table*}[t]
\resizebox{\linewidth}{!}{
    \centering
    \begin{tabular}{|c|c|c|c|}
    \hline
         \textbf{Generated Transcription} & \textbf{True Transcription} & $W_{acc}$ & $C_{acc}$\\
         \hline
         after that it was easy to forget actually to forget & after that it was easy to forget actually to forget & 100.0 & 100.0 \\
         \hline
         you haven t seen any of them no she & you haven t seen any of them no sir & 88.89 & 94.29 \\
         \hline
         that he will teach me a few tricks when water is coming & yet he will teach you a few tricks when morning is come & 66.67 & 70.91 \\
         \hline
         at the same time every avenue of the home was felt in his voice & at the same time every avenue of the throne was assaulted with gold & 61.54 & 73.13 \\
         \hline
        he had broken into the straight line & he had broken into her courtyard & 50.0 & 56.25 \\
         \hline
         oh sir what s different observed joseph arching and beneath it & oh say that s different observed markham altering his demeanor & 30.0 & 61.29 \\
         \hline
         her consciousness of her was now in order & his constancy to her was now rewarded & 28.57 & 54.05 \\
         \hline
         you ve got a bit of what wasn t his kind doing in there mister & you ve got a birthday present this time jim and no mistake & 8.33 & 46.55 \\
         \hline
    \end{tabular}
    }
    \caption{Sample transcriptions generated by {\papertitle} compared to the original utterances from the LibriSpeech dataset, illustrating the system's performance in noisy radar-audio conditions, along with their word accuracy rate ($W_{acc}$) and character accuracy rate ($C_{acc}$).}
    \label{tab:utterances_table}
\end{table*}
